Model-based design of temporal analysis of products (TAP) reactors: A simulated case study in oxidative propane dehydrogenation

Temporal analysis of products (TAP) reactors enable experiments that probe numerous kinetic processes within a single set of experimental data through variations in pulse intensity, delay, or temperature. Selecting additional TAP experiments often involves arbitrary selection of reaction conditions or the use of chemical intuition. To make experiment selection in TAP more robust, we explore the efficacy of model-based design of experiments (MBDoE) for precision in TAP reactor kinetic modeling. We successfully applied this approach to a case study of synthetic oxidative propane dehydrogenation (OPDH) that involves pulses of propane and oxygen. We found that experiments identified as optimal through the MBDoE for precision generally reduce parameter uncertainties to a higher degree than alternative experiments. The performance of MBDoE for model divergence was also explored for OPDH, with the relevant active sites (catalyst structure) being unknown. An experiment that maximized the divergence between the three proposed mechanisms was identified and led to clear mechanism discrimination. However, re-optimization of kinetic parameters eliminated the ability to discriminate. The findings yield insight into the prospects and limitations of MBDoE for TAP and transient kinetic experiments.

==> extra.tex <==
\section{Results and discussion}

\subsection{Methodology}

%\begin{equation}\label{PDE-form-gas}
%	 \varepsilon{}\frac{\partial C_{i}(x,t)}{\partial t} - \frac{\partial}{\partial x}\cdot{}(D_{i}\;{}\nabla{}C_{i}(x,t)) = R_{i}
%\end{equation}

%\textcolor{blue}{[GSG] in the KINNs notation, $\mathbf{c}=[c_i]^T$, with $\partial_t\mathbf{c}=\dot{\mathbf{c}}$ and $\partial_x\mathbf{c}=\mathbf{c}'$, $\mathbf{M}$ is the stoichiometry matrix, $\mathbf{r}$ a vector with rates of reaction, and $\mathbf{d}=[D_i]^T$, we would have
%proposed notation: $x_i$ scalar element of $\mathbf{x}$ vectors, $\mathbf{X}$ denotes matrices.\\
%}
%where the void fraction is defined as $\varepsilon{}$, the concentration of gas $i$ at length $x$ and time $t$ is, the Knudsen diffusion of gas $i$ is $D_{i}$, and the lumped rate term involving species $i$ is $R_{i}$. 

%\begin{equation}\label{flux_eq}
%    F_{i} = D_{i}\frac{\partial C_{i}(L,t)}{\partial x}
%\end{equation}
%\textcolor{blue}{[GSG] With the notation above and $\mathbf{f}=[F_i]^T\in\mathcal{R}_+^{G}$,

%where the synthetic and observed outlet fluxes of gasses $G$ and time points $\tau{}$ are defined as $\hat{F}_{i,j}$ and $F_{i,j}$, respectively. 

%where $L$ is the length of the TAP reactor and $F_{i}$ is the outlet flux of species $i$. When fitting TAP experimental data with PDEs, it is also necessary to define the objective function,

%\begin{equation}
%\label{objectiv_function_std}
%    J^{N} = \mathlarger{\sum^{G}_{i=1}}\mathlarger{\sum^{\tau}_{j=1}}  \frac{(\hat{F}_{i,j} - F_{i,j})^{2}}{2\hat{\sigma{}}_{i,j}^{2}}   
%\end{equation}

%\textcolor{blue}{[GSG] Here the notation might become a bit convoluted if we lump the number of reactions in $\mathbf{f}$ (vector), i.e. introducing an error for a timepoint $j$ as 

%\begin{equation}
%\label{objectiv_function_std}
%    J^{N} = \mathlarger{\sum^{G}_{i=1}}\mathlarger{\sum^{\tau}_{j=1}}  \frac{(\hat{F}_{i,j} - F_{i,j})^{2}}{2\hat{\sigma{}}_{i,j}^{2}}   
%\end{equation}

%\textcolor{blue}{[GSG] Here the notation might become a bit convoluted if we lump the number of reactions in $\mathbf{f}$ (vector), i.e. introducing an error for a timepoint $j$ as \boldsymbol{\varepsilon}_{j}=\hat{\mathbf{f}}_j-\mathbf{f}$

%\begin{equation}
%    \mathbf{H}^{N}_{\theta} = \frac{ \partial{}^{2} J^{N} } {\partial{\theta{}}^{2}} 
%\end{equation}

%\begin{equation}\label{dynamicSensitivity}
%   Q_{g} = \begin{bmatrix}
%     \left.\frac{\partial{}\hat{F}_{g}}{\partial{}\theta{}}\right\rvert_{\textrm{t}} & ... & \left.\frac{\partial{}\hat{F}_{g}}{\partial{}\theta{}_{\phi}}\right\rvert_{\textrm{t}}\\
%   ... & ... & ...\\
% \left.\frac{\partial{}\hat{F}_{g}}{\partial{}\theta{}}\right\rvert_{\tau{}} & ... & \left.\frac{\partial{}\hat{F}_{g}}{\partial{}\theta{}_{\phi}}\right\rvert_{\tau{}}
% \end{bmatrix}
% \end{equation}  

\subsection{Outline}

The document layout should follow the style of the journal concerned.
Where appropriate, sections and subsections should be added in the
normal way. If the class options are set correctly, warnings will be
given if these should not be present.

\subsection{References}

The class makes various changes to the way that references are
handled.  The class loads \textsf{natbib}, and also the
appropriate bibliography style.  References can be made using
the normal method; the citation should be placed before any
punctuation, as the class will move it if using a superscript
citation style
\cite{Mena2000,Abernethy2003,Friedman-Hill2003,EuropeanCommission2008}.
The use of \textsf{natbib} allows the use of the various citation
commands of that package: \citeauthor{Abernethy2003} have shown
something, in \citeyear{Cotton1999}, or as given by
Ref.~\citenum{Mena2000}.  Long lists of authors will be
automatically truncated in most article formats, but not in
supplementary information or reviews \cite{Pople2003}. If you
encounter problems with the citation macros, please check that
your copy of \textsf{natbib} is up to date. The demonstration
database file \texttt{achemso-demo.bib} shows how to complete
entries correctly. Notice that ``\latin{et al.}'' is auto-formatted
using the \texttt{\textbackslash latin} command.

Multiple citations to be combined into a list can be given as
a single citation.  This uses the \textsf{mciteplus} package
\cite{Johnson1972,*Arduengo1992,*Eisenstein2005,*Arduengo1994}.
Citations other than the first of the list should be indicated
with a star. If the \textsf{mciteplus} package is not installed,
the standard bibliography tools will still work but starred
references will be ignored. Individual references can be referred
to using \texttt{\textbackslash mciteSubRef}:
``ref.~\mciteSubRef{Eisenstein2005}''.

The class also handles notes to be added to the bibliography.  These
should be given in place in the document \bibnote{This is a note.
The text will be moved the the references section.  The title of the
section will change to ``Notes and References''.}.  As with
citations, the text should be placed before punctuation.  A note is
also generated if a citation has an optional note.  This assumes that
the whole work has already been cited: odd numbering will result if
this is not the case \cite[p.~1]{Cotton1999}.

\subsection{Floats}

New float types are automatically set up by the class file.  The
means graphics are included as follows (Scheme~\ref{sch:example}).  As
illustrated, the float is ``here'' if possible.
\begin{scheme}
  Your scheme graphic would go here: \texttt{.eps} format\\
  for \LaTeX\, or \texttt{.pdf} (or \texttt{.png}) for pdf\LaTeX\\
  \textsc{ChemDraw} files are best saved as \texttt{.eps} files:\\
  these can be scaled without loss of quality, and can be\\
  converted to \texttt{.pdf} files easily using \texttt{eps2pdf}.\\
  %\includegraphics{graphic}
  \caption{An example scheme}
  \label{sch:example}
\end{scheme}

\begin{figure}
  As well as the standard float types \texttt{table}\\
  and \texttt{figure}, the class also recognises\\
  \texttt{scheme}, \texttt{chart} and \texttt{graph}.
  \caption{An example figure}
  \label{fgr:example}
\end{figure}

Charts, figures and schemes do not necessarily have to be labelled or
captioned.  However, tables should always have a title. It is
possible to include a number and label for a graphic without any
title, using an empty argument to the \texttt{\textbackslash caption}
macro.

The use of the different floating environments is not required, but
it is intended to make document preparation easier for authors. In
general, you should place your graphics where they make logical
sense; the production process will move them if needed.

\subsection{Math(s)}

The \textsf{achemso} class does not load any particular additional
support for mathematics.  If packages such as \textsf{amsmath} are
required, they should be loaded in the preamble.  However,
the basic \LaTeX\ math(s) input should work correctly without
this.  Some inline material \( y = mx + c \) or $ 1 + 1 = 2 $
followed by some display. \[ A = \pi r^2 \]

It is possible to label equations in the usual way (Eq.~\ref{eqn:example}).
\begin{equation}
  \frac{\mathrm{d}}{\mathrm{d}x} \, r^2 = 2r \label{eqn:example}
\end{equation}
This can also be used to have equations containing graphical
content. To align the equation number with the middle of the graphic,
rather than the bottom, a minipage may be used.
\begin{equation}
  \begin{minipage}[c]{0.80\linewidth}
    \centering
    As illustrated here, the width of \\
    the minipage needs to allow some  \\
    space for the number to fit in to.
    %\includegraphics{graphic}
  \end{minipage}
  \label{eqn:graphic}
\end{equation}

\section{Experimental}

The usual experimental details should appear here.  This could
include a table, which can be referenced as Table~\ref{tbl:example}.
Notice that the caption is positioned at the top of the table.
\begin{table}
  \caption{An example table}
  \label{tbl:example}
  \begin{tabular}{ll}
    \hline
    Header one  & Header two  \\
    \hline
    Entry one   & Entry two   \\
    Entry three & Entry four  \\
    Entry five  & Entry five  \\
    Entry seven & Entry eight \\
    \hline
  \end{tabular}
\end{table}

Adding notes to tables can be complicated.  Perhaps the easiest
method is to generate these using the basic
\texttt{\textbackslash textsuperscript} and
\texttt{\textbackslash emph} macros, as illustrated (Table~\ref{tbl:notes}).
\begin{table}
  \caption{A table with notes}
  \label{tbl:notes}
  \begin{tabular}{ll}
    \hline
    Header one                            & Header two \\
    \hline
    Entry one\textsuperscript{\emph{a}}   & Entry two  \\
    Entry three\textsuperscript{\emph{b}} & Entry four \\
    \hline
  \end{tabular}

  \textsuperscript{\emph{a}} Some text;
  \textsuperscript{\emph{b}} Some more text.
\end{table}

The example file also loads the optional \textsf{mhchem} package, so
that formulas are easy to input: \texttt{\textbackslash ce\{H2SO4\}}
gives \ce{H2SO4}.  See the use in the bibliography file (when using
titles in the references section).

The use of new commands should be limited to simple things which will
not interfere with the production process.  For example,
\texttt{\textbackslash mycommand} has been defined in this example,
to give italic, mono-spaced text: \mycommand{some text}.

\section{Extra information when writing JACS Communications}

When producing communications for \emph{J.~Am.\ Chem.\ Soc.}, the
class will automatically lay the text out in the style of the
journal. This gives a guide to the length of text that can be
accommodated in such a publication. There are some points to bear in
mind when preparing a JACS Communication in this way.  The layout
produced here is a \emph{model} for the published result, and the
outcome should be taken as a \emph{guide} to the final length. The
spacing and sizing of graphical content is an area where there is
some flexibility in the process.  You should not worry about the
space before and after graphics, which is set to give a guide to the
published size. This is very dependant on the final published layout.

You should be able to use the same source to produce a JACS
Communication and a normal article.  For example, this demonstration
file will work with both \texttt{type=article} and
\texttt{type=communication}. Sections and any abstract are
automatically ignored, although you will get warnings to this effect.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% The "Acknowledgement" section can be given in all manuscript
%% classes.  This should be given within the "acknowledgement"
%% environment, which will make the correct section or running title.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> purge.tex <==
% Results

As noted in the methodology, the selection of initial conditions for TAP experiments can be arbitrary or come from the users chemical intuition. For this reason, we choose an arbitrary set of initial conditions as our initial experiment. The temperature is selected as 700 K and the pulse intensity for each reactant species is also defined as 1 nmol. No delay is included in the initial optimization, either. The optimized parameters for this initial condition, as well as the uncertainty of the system, are presented in Table \ref{opdh_initial_fit_table}. A visual of the optimal fit is also presented in Figure \ref{opdh_initial_fit_precision}. 

Upon optimization, we observe most of the parameters have strong agreement with the values in Table \ref{opdh_model_precision}. Although many of these parameters match the actual values, some still have a high degree of uncertainty associated with them (95\% confidence intervals approximately equal to $5 \cdot 10^{-2}$ eV). Of the parameters, $\Delta{}G^{1}$ and $G_{a}^{4}$ (which represent the Gibbs free energy of adsorption of propane and the free energy of activation of propane combustion, respectively) have the lowest degrees of uncertainty with values approximately equal to $2 \cdot 10^{-3}$ eV (meaning propane is the dominant species in the system, and combustion is the most active reaction). The parameter with the least accurate fit was $\Delta{}G^{2}$ (i.e. the free energy of dissociative adsorption of oxygen), with an approximate uncertainty of $1 \cdot 10^{-1}$ eV. The $\Delta{}G^{2}$ value also diverges from the actual value by about 0.15 eV. This is likely the result of the influence of other parameters masking the relevance of $\Delta{}G^{2}$ through the rapid consumption of the pulsed in oxygen. Since the signal is low for oxygen, it is difficult to extract quantitative details from the experiment for this parameter.

\subsubsection{Identifying additional experiments}
Following the initial optimization, we explored the inclusion of additional experimental data at alternative operating conditions. For the grid search of initial conditions explored, we included delays up to 0.6 seconds for $C_{3}H_{8}$, temperatures between 650 and 700 K, and pulse intensities for $C_{3}H_{8}$ and $O_{2}$ between 1 and 2 nmol. After we fitted the kinetic model to our arbitrary initial experimental data set, we can use the extracted parameters and their associated uncertainties to identify an appropriate secondary experiment with MBDoE. As noted in the methodology section, we use a grid search to explore the initial conditions of interest. The grid involves the propane and oxygen pulse intensities 1, 1.5, and 2 nmol, the reactor temperatures 650, 675, and 700K, and the the propane pulse delays 0, 0.15, 0.3, 0.45, and 0.6 s. Once each of these experiments was specified, we used Equations \ref{dynamicSensitivity} and \ref{fisherInformationMatrix} to construct the Fisher information matrix. In other words, we generated dynamic sensitivity data at each point and converted that, along with the prior covariance matrix, into a single matrix. Heat maps of this process are presented in Figure \ref{mbdoe_heatmap}. Trends in each of the initial conditions are observable between and within each of the subplots, with lighter colors indicating less useful experiments (higher D values) and darker colors indicating more useful experiments (lower D values). 

Within each of the 8 subplots are the 9 combinations of propane and oxygen pulse intensities. When increasing each simultaneously or independent of each other, an improvement in predicted experiment utility is observed. This trend is found for all delay and temperature variations without exception. Based on the initial model, experiments with the maximum pulse intensities should result in the most improved model. This is intuitive, since larger pulse intensities will amplify the signal-to-noise ratio and suggests that in general TAP experiments should be run with the largest practical pulse intensities that do not violate the Knudsen diffusion or isothermal assumptions.

Each row of the subplots is associated with variations in the delay of propane, with the top row representing no delay and the bottom row representing 0.45 seconds. The change in experiment impact with delay is sharpest initially between 0 and 0.15 seconds, indicating that it is important to include at least some delay in the propane pulse to increase experiment utility. Increasing the delay in 0.15 second increments does result in a shift in parameter improvement, but it is subtle enough to require close inspection of the plots. 

Temperature selection was also found to have a noticeable impact on experiment value. In Figure \ref{mbdoe_heatmap}, each column represents the temperatures (from left to right) 675 and 700 K. Between the two, a temperature of 675 K consistently outperforms the 700 K experiments. The strongest contrast between the temperatures when looking at pulse delays also occurs at a pulse delay of 0.

Of the secondary experiments explored in the grid search, the experiment that provided the least additional value was at 700 K, 1 nmol pulse intensity of propane and oxygen, and no delay in either gas. This is an expected result, since it is identical to the initial experiment and would express all reaction processes to the same degree. The predicted optimal experiment followed the trends outlined in this section with a temperature of 650 K, 2 nmoles of both propane and oxygen, and a delay of 0.45 seconds for propane. 

\begin{figure}[H]
    \centering 
  \includegraphics[width=11cm]{2_results/images/mbdoe_heatmap.pdf}
  \caption{Heat maps showing a subsubsection of the grid search performed to identify the best secondary experiment using the MBDoE and D-optimality criteria, as well as the current understanding of the uncertainty found in initial optimization.}
  \label{mbdoe_heatmap}
\end{figure}

\subsubsection{Correlation of experiment value with predicted experiment value}

After sampling over the initial condition space and re-optimizing the parameters based on the secondary experiments, the A, D, and E-optimal criteria were calculated to determine the adequacy of their predictive ability. As an indicator of the quality of the reoptimized parameters, the trace, determinant, and largest eigenvalue of the covariance of the re-fitted parameters was used (here referred to as the actual A, D, and E-values). The MBDoE is typically validated and applied to systems with few parameters (e.g. two). When one or two parameters are used, it is easy to visualize the uncertainty associated with a system, since confidence ellipsoids can be drawn in the parameter space. As mentioned earlier in the chapter, the A, D, and E-values have a geometrically meaningful interpretation. In the case of the confidence ellipsoid, the A-value would represent the area of a box drawn around the ellipse, the D-value would represent the area of ellipse itself, and the E-value would represent the length of the major axis of the ellipse \cite{franceschini2008model}. When an optimal experiment is identified, the parameters optimized to the new experiment, and the uncertainty recalculated, the prior and new confidence ellipsoid can be plotted together. If the ellipsoid for the new experiment falls within the old ellipsoid, then the experiment can be labeled a success. If it is approximately the same size, it can be seen as having had little impact on the certainty of the mechanism. When looking at a higher number of parameters in a system, relying on this visual is infeasible and quantitative alternatives must be used. Using the A, D, or E-values for the actual, instead of the predicted, covariance matrix should help us draw conclusions without relying on multi-dimensional visualizations.

The A-optimality, which represents the trace of the predicted Fisher information matrix, was first used as a possible indicator of optimality, and is presented in the first column of Figure \ref{optimal_criteria}. In these subplots, there is little correlation between the predicted A-value and these criteria, with the lowest A-values having average performance (e.g. falling in-between the distribution of possible confidence intervals). If the A-optimal was blindly used, a decent experiment would be predicted, but the potential for future utility seems muted due to the lack of correlation observed.

Next, the D-optimal value was used as a predictive metric for the actual D-value and is presented in the middle column of Figure \ref{optimal_criteria}. In this case, a strong correlation was observed, with low values of the predicted D aligning with low values of the actual D-value. Although there is still dispersion in actual D-values along the predicted D-value, it is narrower than that of the A-optimal and it is also relatively consistent. The lowest predicted D-value does not predict the exact lowest actual D-value, but it is within the order of magnitude of the lowest and outperforms a majority of the competing experiments. At the opposite end of the spectrum, the highest predicted D-value aligns with the highest actual D-value. When using the A and E-values to evaluate the new experiment at the actual local minimum, a similar lack of correlation is observed to that of the predicted A-value plots.

Last, we explored the use of the E-value as a predictive metric. The E-value represents the highest eigenvalue in the Fisher information matrix and minimizing it should reduce the uncertainty of the least understood parameter. The E-value is plotted against the various evaluation criteria in the third column of Figure \ref{optimal_criteria}. The trends in E-value and A-value are nearly identical, with only mild horizontal shifts in the values. It is clear that neither the A or E-values perform well in predicting a quality experiment and D-optimal values should be used in their place. 

\begin{figure}[H]
    \centering 
  \includegraphics[width=16cm]{2_results/images/ade_criteria.pdf}
  \caption{Scatter plots showing the connection between the predicted A, D, and E-optimality and the explicit A, D, and E-values of the refitted mechanism covariance matrix. }
  \label{optimal_criteria}
\end{figure}

Now that the D-optimal was identified as the preferred selection criteria, it is important to observe the ways in which each of the initial conditions impact the extracted information. Again, the intensity and delay of propane, the intensity of oxygen, and the reactor temperature were explored in experiment selection. The D-optimal plot presented in Figure \ref{optimal_criteria} is again presented in Figure \ref{optimal_criteria_initial_conditions}, but through the lens of each initial condition. Subplot A of Figure \ref{optimal_criteria_initial_conditions} highlights the impact the pulse intensity of propane has on the prediction. Although the trend observed in the heat maps is maintained, there is significant overlap between each of the propane intensities. The highest propane pulse intensity generally out performs the lower intensities, but not always, with some 1 nmol pulses beating 2 nmol pulses. This indicates propane pulse intensity is not the single deciding factor driving experiment selection. 

Subplot B in Figure \ref{optimal_criteria_initial_conditions} shows the D-optimal variation with respect to the pulse intensity of oxygen. The trend in oxygen pulse intensity follows that of propane, with higher intensities generally resulting in better performing experiments. Again, there is overlap between these intensity domains, and some of the lower intensity values eclipse those of the high intensities. The predicted correlation found in the previously discussed heat maps stands and maximizing the intensity for both gasses leads to higher precision in the parameters. 

Subplot C in Figure \ref{optimal_criteria_initial_conditions} shows the D-optimal variation with respect to the delay in propane. Unlike the trends observed for pulse intensities, the trends in delay are more diverse between values. When no delay is included (pulse delays of zero), the strongest correlation between the predicted and actual D-values was observed of any of the subplots (indicating the current model has the ability to identify quality experiments with no delay, but not the ability to predict optimal experiments with delay). Very little dispersion is observed in the actual D-values along the predicted D-values. The prediction of experiments with a delay, however, are more dispersed and complicated to describe a general trend for. The dispersion of predicted D-Values between 0.15 and 0.6 seconds overlap with one another. In other words, the lowest and highest D-values for each of the values of delay are approximately the same. The dispersion of the actual D-values still overlaps, but to a less pronounced degree. Delays of only 0.15 seconds under-perform (have higher actual D-values) than higher delays. The delays of 0.3, 0.45, and 0.6 seconds do have a stronger overlap however, and varying between these values seems to have less impact. Again, the model previously defined is adequately able to predict optimal experiments with similar operating conditions, but the inclusion of more complex conditions can limit its predictability. 

\begin{figure}[H]
    \centering 
  \includegraphics[width=16cm]{2_results/images/paper_fig_2 (1).pdf}
  \caption{The scatter plots between the predicted and actual D-values through the lens of propane delay, propane and oxygen pulse intensity, and the reactor temperature.}
  \label{optimal_criteria_initial_conditions}
\end{figure}

Last, the impact of reactor temperature on the D-value is presented in subplot D of Figure \ref{optimal_criteria_initial_conditions}. Again there is strong overlap between each of these classifications, but it varies in its orientation from that of the intensity overlaps. Here the predicted D-values generally favor lower temperatures, with the highest and lowest D-values for 650 K falling to the left of the associated D-values of 675 and 700 K. However, the actual D-values favor the opposite trend by a narrow margin, with the lowest values for 675 and 700 K falling noticeably below that of 650 K. Unlike the intensity trend, the best trend in temperature is not captured by the MBDoE, indicating the MBDoE to identify the optimal experiment in an operating condition grid.

Now that trends based on initial conditions have been observed, the impact the optimal criteria have on reducing parameter uncertainties following reoptimization at each experiment, instead of all simultaneously in the D-optimal form, can be observed. These plots are presented in Figure \ref{optimal_std}, with the confidence interval of the re-fitted parameter being presented on the y-axis. As a visual reference, the previously generated D-optimal actual distribution is provided in the upper left subplot. The upper right subplot shows the confidence intervals around the refitted values of $\Delta{}G_{0}$, or the free energy of adsorption of propane. Although the lowest uncertainty is not observed at the lowest D-value, the D-optimal experiment is outperforming the majority of the competing experimental designs. The general downward trend of D-values is also observed, indicating the design does yield the correct general trend for this parameter. Next, the free energy of adsorption of oxygen was explored. Unlike $\Delta{}G_{0}$and many of the other parameters, there is no trend in this distribution and the ``optimal'' experiment only leads to an average reduction in uncertainty. The uncertainty in some of the experiments even falls above the previously found uncertainty, indicating this parameter is poorly defined in the system and other parameters dominate the experimental search. Even though some experiments do cause a dramatic reduction in uncertainty, they are predicted to be mediocre experiments and other experiments with slightly different predicted D-values fall far above them. This indicates that the MBDoE does not work equally well for all parameters, and may heavily favor parameters that are already well defined. However, the D-optimal experiment does still reduce the uncertainty, even for poorly-defined parameters. After $\Delta{}G_{1}$, the activation of adsorption of oxygen ($Ga_{1}$)  was explored and the uncertainty reduction observed in $\Delta{}G_{0}$ is again observed. Unlike the previous trend, a few experiments perform far worse than competing ones. However, these all fall at high predicted D-values and even though the logarithmic trend is not maintained, these experiments would be rejected. Next, the free energy of adsorption of propene ($\Delta{}G_{2}$) was analyzed and is presented in subplot E. Of the parameters discussed so far, this parameter is the least impacted by the initial condition, although gradual reduction in the uncertainty is still observed as the D value decreases. Some experiments result in little to no change in the uncertainty, but a majority of them reduced the uncertainty a factor of 2-3.

The free energies of activation of propane dehydrogenation, propane combustion, and propene combustion ($G_{a}^{3}$,$G_{a}^{4}$, and $G_{a}^{5}$, respectively) are presented in in the final subplots. No outliers or surprises are found in these trends. There is the same general improvement in the uncertainties found in the other figures with a few exceptions at experiments predicted to perform poorly. The MBDoE therefore performs well for these parameters. 

\begin{figure}[H]
    \centering 
  \includegraphics[width=14cm]{2_results/images/paper_fig1.pdf}
  \caption{Scatter plots between the standard deviation of the free energy parameters and the predicted D-value. The confidence interval based on the initial experiment only is the black horizontal line in the plot.}
  \label{optimal_std}

\end{figure}

\subsubsection{Additional MBDoE-based experiment selection}

Now that an initial experiment was found to significantly reduce the uncertainty of a majority of the experiments, an additional step should be taken to determine if further uncertainty reductions can be made. In this workflow, we will again run the MBDoE experiments to identify the next best experiment using the kinetic parameters and covariance found from the prior experiments. Again we will re-optimize the parameters and quantify the uncertainty at all of the experimental conditions used in the initial condition space, providing us with information related to general trends and the overall utility of the uncertainty.

As was done with the previous MBDoE application, we first look at the predictions found through the MBDoE, which are visualized in Figure \ref{ternary_variation}. Much like the previous experiment exploration, high intensities were favored for both propane and oxygen pulses for all temperature and delay combinations. The temperature variation in predicted optimal experiment also resembled the original experiment selection, with the experiments involving 700 K expected to significantly under-perform compared to 650 and 675 K. The only initial condition to see a noticeable shift compared to the original analysis was the pulse delay. Instead of maintaining a trend of higher delay resulting in more ideal experiments, lower values of delay are preferred. The predicted value in an experiment with no delay in propane is still found to be low, but the 0.15 second delay in propane is found to be the ideal experiment. With all of this considered, the optimal experiment was found to be at 650 K with 2 nmol pulses of propane and oxygen, and a 0.15 second delay in propane. 

To explore the performance of this additional application of MBDoE, similar graphs to those of Figure \ref{optimal_std} were generated and are presented in Figure \ref{ternary_variation}. Subplot A again shows the direct comparison between the actual and predicted D-values for each experiment. Unlike the predicted D-value plot found for the first additional experiment, there is far more vertical dispersion along the predicted values. The optimal predicted experiment also only provides a mild improvement in the model compared to alternative ones, indicating there is less added benefit to the experiment. There are also more experiments that perform similarly or out perform the predicted optimal. The results reveal even more outliers when analyzed in terms of the individual parameter uncertainties. A few of the parameters ($Ga_{1}$, $\Delta{}G_{2}$, and $Ga_{5}$) do maintain a gradual uncertainty reduction as the D-value decreases. However, other parameters fair worse and have disjointed variations in their actual D-values. $\Delta{}G_{0}$ and $Ga_{3}$ are two examples of this, each having sparse and lower actual D-values in the region with highest predicted D-value. Worst of all is the performance of $\Delta{}G_{1}$, our poorest defined parameter in the system based on our prior analysis. Although there are some experiments that have low predicted and actual D-values simultaneously, the distribution outside of these few has limited correlation. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We begin by performing a grid search over the initial condition space specified in the Section \ref{chpt5:intro}. This grid search consists of generating the synthetic experimental data from the black-box (i.e. a noisy TAP simulation) under each set of initial conditions. Initially, the synthetic experimental data is generated with the exact mechanisms and their kinetic parameters introduced in the methodology section of this chapter, i.e. we use the same parameter values between the data generation (black-box) and the predicted simulation, and noise is only added to the resulting fluxes, corresponding to the case where both experiments are performed in the same TAP setup (e.g. a multi-pulse experiment with the same packed bed). Subsequently, we perform the same set of simulations, but perturb the kinetic parameters slightly for each simulation, corresponding to noise in the underlying kinetic parameters due to minor variations in catalyst loading/chemistry between experiments (e.g. the case where the TAP reactor is re-loaded in between experiments).

To study a broader range of scenarios for mechanism divergence, we used each of the three mechanisms to generate experimental data sets, corresponding to three different possible ``real'' scenarios. This will help determine the validity and flexibility of MBDoE for divergence more effectively than exploring data generated from a single mechanism. Figure \ref{det_div} shows this analysis for both the deterministic (left column) and the uncertain (right column) definitions of the divergence criteria for each of the three models under the three different scenarios. 

First, the deterministic criteria shows very clear trends of increasing the incorrect mechanism's BIC values near higher values of predicted divergence, effectively increasing the separation between the correct and incorrect models. When mechanism 1 is used to generate the experimental data, the BIC values of mechanism 2 and 3 increase linearly at approximately the same rate. When mechanism 2 is used to generate the experimental data set, the BIC for mechanism 3 is approximately constant throughout and the BIC value of mechanism 1 gradually increases with the predicted divergence. Last, when mechanism 3 is used for the data generation, the BIC values for mechanism 1 and 2 overlap significantly at low divergence but gradually spread apart at higher values. It should also be noted how distinguishable this example, as well as BIC values uncertainty criteria figures to the right, are in terms of mechanism selection. A general conclusion can be made that any experiment can be performed and the correct mechanism will be identified, highlighting the utility of the TAP system even in the absence of experimental design. 

When looking at the uncertainty based divergence criteria (right column of Figure \ref{det_div}), we see the same general increase in BIC values, but observe a less continuous pattern than the deterministic criteria. Instead of smooth increases that were observed in the deterministic version, we see some clusters with high BIC values that have low predicted divergence values. There also appear to be individual clusters of experiments breaking the trend, indicating that the increase in uncertainty is a result of a unique initial condition. This trend is only occurring for the mechanisms that are not used to generate the experimental data (with the correct mechanism again falling flat with inaccuracies only occurring due to noise present in the experimental simulation). Although there are differences between the predictions in each divergence criteria, the correct mechanism is easily and accurately found with any experiment selection.

When variations in the mechanism kinetic parameters are included, differences in the simulations predicted with divergence criteria are less clear cut and depend more on the initial conditions selected. The divergence and BIC value analysis is visualized in Figure \ref{unc_div}, with the deterministic and uncertain divergence criteria being provided in the left and right columns, respectively. When the experimental data is generated with mechanism 1 and 3, similar trends to those observed in Figure \ref{det_div} (i.e. the experimental data without the parameter variations) are observed. The only difference between the two experimental data generation processes for the mechanism with and without noise is the increase in the BIC value for the correct mechanism. However, these increases are not enough to make the mechanism indistinguishable. However, when mechanism 2 is used to generate the experimental data, the ability to distinguish the mechanisms without identifying an appropriate experiment becomes more challenging. The BIC values of mechanism 3 are far above those of the the other two (i.e. mechanism 3 will not describe the experimental data well), but the BIC values for mechanisms 1 and 2 overlap significantly at low values of the divergence criteria. For the deterministic based approach, the same linear increase is observed and higher divergence values do correlate with more distinguishability in mechanism 2. The same to a certain degree can be said for the uncertainty-based divergence, where high BIC variation is observed at higher predicted divergence. Much like the use of the exact parameters experimental data generation, outlier clusters of high BIC distinguishable experiments are found at low divergence values. The conclusion is that not all experiments would be able to identify the correct mechanism, but the MBDoE approach outlined here is capable of identifying an experiment that identifies the correct mechanism regardless of which divergence criterion is used. 

%% Maximum divergence

\begin{figure}[H]
    \centering 
    \hspace*{-2cm}
  \includegraphics[width=16cm]{2_results/images/divergence_det_plots.pdf}
  \caption{The results of the divergence based grid search in the TAP experimental condition space with no variations in the experimental data generation model. The columns represent each divergence criteria used (deterministic and uncertain based), while the rows represent each of the models used to generate the experimental data (Mechanism 1, 2, and 3).}
\label{det_div}
\end{figure}

The least useful experiment identified for the deterministic and uncertain based divergence were identical and involved a temperature of 650 K, pulse intensities of 0.5 nmol of propane and oxygen, and no delay of either gas. The optimal experiment when using the deterministic divergence criteria was a temperature of 750 K, a pulse intensity of 0.5 nmol of propane, a pulse intensity of 2 nmol of oxygen, and a delay of 0.45 s of propane. The uncertainty based divergence optimal experiment was the same as deterministic based criteria, with the exception of the temperature being 700 K instead of 750 K. The outlet flux visuals of propane, oxygen, propene, water, and carbon dioxide for the lowest predicted divergence, the deterministic optimal, and the uncertainty optimal experimental conditions are presented in Figures \ref{flux_worst}, \ref{flux_det_pre}, and \ref{flux_det_pre}, respectively. These visuals clearly show the reason mechanism 3 was predicted to consistently be incompatible with the experimental data, where none of the outlet flux predictions (with exception to the products water and carbon dioxide), have any semblance of consistency with the experimental data. Mechanism 1 and 2, however, strongly overlap with one another. The experiment predicted to have the lowest divergence actually does maintain a low degree of visual divergence. Each of the outlet flux curves, with the exception of the oxygen, is enveloped in the noisy experimental data. Both of the oxygen simulations fall outside of the experimental data, but they appear to symmetrically diverge above and below it. 

The predicted maximum deterministic based divergence criteria has similar trends to the worst experiment, with the exception of oxygen simulation again diverging from the experimental data. The intensity of the experimental oxygen is approximately twice as high as the least informative experiment, with the second mechanism scaling to a similar degree and the first mechanism staying approximately the same. The ability to distinguish the mechanisms even appears more challenging for this experiment, since the signal to noise ratio is lower for propane and propene. Based on these results, the oxygen simulation appears to drive the deterministic divergence criteria. The predicted maximum uncertainty based divergence criteria does appear to have higher degree of visual divergence. Oxygen follows the same trend as the predicted maximum deterministic based divergence experiment, but experiences a lower general intensity. Propane and propene again overlap to the same degree as the previous experiments and get lost in the noise, but water and carbon dioxide do begin diverging more. The first mechanism actually appears to follow the experimental data better than the second mechanism, with the intensities found in mechanism 2 being smaller. 

\begin{figure}[H]
    \centering 
    \hspace*{-2cm}
  \includegraphics[width=10cm]{2_results/images/0_0_0_0.pdf}
  \caption{The experiment with the lowest predicted divergence using the deterministic and uncertainty based criteria. The reactor temperature is 650 K, the pulse intensities are 0.5 nmol for both propane and oxygen, and the delay in propane is 0 seconds. Mechanism 1, 2, and 3 are shown with solid blue, dashed green, and dotted gold lines, while the experimental data is shown with black dots.}
\label{flux_worst}
\end{figure}

\begin{figure}[H]
    \centering 
    \hspace*{-2cm}
  \includegraphics[width=10cm]{2_results/images/0_3_3_4.pdf}
  \caption{The experiment with the optimal predicted divergence using the deterministic based criteria. The reactor temperature is 750 K, the pulse intensity of propane is 0.5 nmol, the pulse intensity of oxygen is 0.5 nmol, and the delay in propane is 0.45 seconds. Mechanism 1, 2, and 3 are shown with solid blue, dashed green, and dotted gold lines, while the experimental data is shown with black dots.}
\label{flux_det_pre}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Discussion

Overall, the MBDoE can be seen as a successful approach, with some caveats. As a first iteration of finding a useful additional experiment, the D-optimal criteria was successful and identified an experiment that performed better than most other experiments. Using this criteria was also relatively robust, since the three or four next best experiments also performed similarly well. These trends were also mostly observed in the individual parameter uncertainties. The parameter uncertainties were consistently reduced with the predicted D-values. However, there was one major exception in $\Delta{}G_{1}$. This parameter had the highest degree of uncertainty of all the parameters following optimization to the initial experiment. Although some trend was observed, the least certain parameter saw limited improvement relative to other experiments at the optimal experiment.

The MBDoE for precision is typically used to reduce the uncertainty in all parameters simultaneously. More specifically, the isolation of individual parameters is rarely used in any step of the search for better experiments. However, we want to determine whether there is any obtainable benefit to this approach when applied to the ternary experiment selection performed in the results section. More specifically, we want to observe a noticeable reduction in the uncertain of our least determined parameter (i.e. $\delta{}G^{1}$). To test this, we performed the MBDoE for precision prediction on a varied combination of parameters to see if better experiments were more accurately predicted. The varied parameter combination actually consisted of the gradual incorporation of less uncertain parameters in the search metric, beginning with only the most uncertain parameter and extending to all of the parameters. These combinations are labeled as A1, A2, A3, etc. for the most uncertain parameter, the two most uncertain parameters, the three most uncertain parameters, etc., respectively. We then looked at the impact these selection criteria had on the standard deviation for each parameter in the system, which is presented in Figure \ref{gradual_mbdoe}. 

The right most column of Figure \ref{gradual_mbdoe} is identical to those of Figure \ref{ternary_variation} in the results section, involving all parameters in the experimental design. As we move leftward along the columns, we begin to see a stronger trend in the observed uncertainties. This trend also isolates certain experiments that inaccurately reduce the uncertainty of some parameters. For example parameter $\Delta{}G_{1}$ in column A1 shows a strong linear trend between the predicted optimal experiment and the true optimal experiment, while also showing a cluster of experiments that fail to follow the trend or lead to better results. $\Delta{}G_{1}$ is again the most uncertain parameter after both the initial and secondary experiments. Although it was reduced to some degree with a ternary experiment, the scatter of the system was broad and an alternative, weaker experiment could easily have been found to be the "ideal" experiment. Although $\Delta{}G_{1}$ is not isolated in the search of the experimental condition space, the Fisher information formulation should lead to the most uncertain parameter driving the search. Isolating the design in terms of $\Delta{}G_{1}$ addresses this issue, having little scatter around the optimal experiments and, in turn, a higher degree of stability and confidence in the result. Simultaneously, the experiments that were found to perform the worst for $\Delta{}G_{1}$ at times lead to the highest certainty for other parameters. More specifically, $\Delta{}G_{0}$ and $Ga_{3}$ had the lowest uncertainty for experiments that were predicted to be the worst for defining $\Delta{}G_{1}$. At these extreme values, other parameters were also found to have higher confidence intervals, indicating a loss in accuracy of the system. The optimal experiment for $\Delta{}G_{1}$ does lead to higher confidence intervals for $\Delta{}G_{0}$ and $Ga_{3}$, but these appear to be more confident values considering the smooth, continuous nature of the trends in all subplots near this region. Focusing the DoE on a single poorly-determined parameter is an effective strategy to reduce the uncertainty on that parameter, especially in the case that the full design of experiments does not significantly reduce uncertainty. We also find that the optimal experiment for one parameter is not always optimal for others, and anti-correlation is possible.

In this case study, we used an exhaustive grid search to determine the utility of MBDoE. This was done to better define our general algorithm for MBDoE with respect to TAP. This approach involves defining the mechanism, fitting and quantifying the uncertainty to an initial, arbitrary experiment, identifying a new experiment based off of MBDoE, and iteratively performing the process until an adequate degree of uncertainty is obtained. If there are parameters that still have unacceptably large error bars then focus on these parameters during the next iteration. The grid search approach should not be seen as the ideal implementation available. Optimization routines that guide the user through the design space instead of testing a predefined set could lead to a lower computational cost and more appropriate experiment. 

Although the MBDoE is able to generally improve the parameters of interest in TAP, exploring more robust methods for experiment selection remains worthwhile. For example, the Bayesian experimental design (BED) has also been used to successfully guide experiments in materials research \cite{wang2021nextorch}. BED avoids the assumption of Gaussian distributions, which is implicit in the MBDoE approach presented here. A fundamental challenge that remains is the efficiency of BED relative to MBDoE. Simulating TAP experiments is costly compared to many kinetic simulations and BED requires a high degree of sampling to be effective \cite{walker2020chekipeuq}. Whether the improvement in experiment selection would outweigh the cost of BED remains unknown. 

Last, pairing TAP state-altering (i.e. multi-pulse) experiments with MBDoE could help further reduce uncertainties on more complex models while gaining a more robust understanding of the materials evolution. Similar to the issue with BED however, running state-altering experiments and performing MBDoE on them is a challenge for multiple reasons. First, the computational cost of multi-pulse fitting can limit the utility of the process, since TAPSolver is currently limited to fitting $<$10 pulses at a time, and multi-pulse experiments typically involve $>$100 pulses. Second, the evolution of the catalyst material could make the analysis infeasible. For example, the complete consumption of one active site could allow a secondary active site to dominate the resulting experimental data, or adsorbate-adsorbate interactions could yield results. that require coverage-dependent kinetic models. Improvements to simulation efficiency that allow fitting of more complex models to significantly larger volumes of data are required to address the challenge of multi-pulse experimental design.

\begin{figure}[H]
    \centering 
    \vspace*{4cm}
    \hspace*{-2cm}
  \includegraphics[width=17cm]{3_discussion/images/parameter_inclusion_design.pdf}
  \caption{MBDoE applied to parameter combinations involving only the most uncertain parameter (A1) and all parameters regardless of parameter uncertainty (A7), with less uncertain parameters being added between them (i.e. A2 through A6). Although not a common approach to MBDoE, the MBDoE based only on the most uncertain parameter ($\Delta{}G_{1}$) in column A appears to significantly outperform those that include most or all of the parameters. This is visible in the confidence intervals being reduced in a stable and predictable manner near low D-values for the predicted experiments.}
  \label{gradual_mbdoe}
\end{figure}

The analysis above shows that MBDoE is capable of identifying experiments with maximal difference, and may be required to identify the correct mechanism, especially in the case where kinetic parameters are expected to vary slightly between experiments. However, the analysis assumes that the rate constants obtained from fitting to the initial experiment are held constant and not re-fitted to the second experiment. In a real scenario, a researcher would likely want to re-fit the model to both experiments to determine whether their kinetic model structure was capable of explaining all the observed data. For this reason, the mechanisms 1 and 2 were re-optimized to the experimental data generated during the grid search. We focus on the mechanism 2 experimental data generated 0.05 eV variations in the free energy parameters. We chose this because it appeared to be the most complex of the scenarios observed. This analysis is presented in Figure \ref{opt_divergence}, with the deterministic and uncertainty based criteria being shown on the left and right subplots, respectively. It is clear that after re-optimization the BIC is not correlated to the divergence, and discriminating between the two mechanisms is not possible at any of the experimental conditions explored. There are some experiments where small differences are observable, but they are scattered randomly throughout the divergence and are too narrow to draw any strong conclusions. The prior optimal experiments for each divergence criteria do not perform well visually either, overlapping entirely with each other and the data. These visuals are provided in Figures \ref{flux_det_opt} and \ref{flux_unc_opt}. These results suggest that the convolution of parametric and structural uncertainty presents a significant challenge, since at least in this case it is not possible to distinguish between mechanisms if the parameters are only obtained by fitting to the kinetic data.  

\begin{figure}[H]
    \centering 
    \hspace*{-1cm}
  \includegraphics[width=17cm]{3_discussion/images/optimized_divergence.pdf}
  \caption{The predicted divergence using the deterministic (left) and uncertainty (right) based criteria compared with the BIC for each mechanism following optimization of the parameters. Far less variation in the BIC between each mechanism is observed and drawing conclusions about the correct mechanism structure is lost.}
\label{opt_divergence}
\end{figure}

\begin{figure}[H]
    \centering 
    \hspace*{-2cm}
  \includegraphics[width=10cm]{3_discussion/images/0_3_3_2_opt.pdf}
  \caption{The experiment with the optimal predicted divergence using the deterministic based criteria following optimization. The reactor temperature is 750 K, the pulse intensity of propane is 0.5 nmol, the pulse intensity of oxygen is 0.5 nmol, and the delay in propane is 0.45 seconds. Mechanism 1 and 2 are shown with solid blue and dashed green, while the experimental data is shown with black dots.}
\label{flux_det_opt}
\end{figure}

==> purged_text_AJ.tex <==
% Abstract

%Although struggling in this case study, the incorporation of surface characterization data or state-altering (i.e. multi-pulse) experiments could help alleviate this challenge and allow investigators to discriminate between proposed mechanisms in a single TAP experiment. 
%MBDoE was generally found to be a valuable tool for alleviating kinetic model uncertainties found in TAP experiments and, with improvements to efficiency, could be a powerful tool in future investigations.

% Introduction
%One reason there are high degrees of uncertainty present in catalytic studies is due to the lack of high-density experimental data set.
%\cite{wellendorff2015benchmark, medford2018extracting, reece2021moving,walker2016uncertainty}. 
%Like other catalytic experimental methods, these uncertainties have seen increased interest over the last decade .
%Additional TAP experimental data sets for kinetic analyses can help further limit the impact of these uncertainties. 
%Although more robust means for selecting experiments are available (e.g. Bayesian experimental design), we believe the MBDoE offers a relatively simple, yet powerful, means for exploring the initial condition space \cite{go2022robust,walker2022bayesian}. 
%Pump-probe TAP experiments, which involve the delayed introduction of a reactant during an experiment. Pump-probe experiments can be a powerful way to selectively express elementary processes within a reaction mechanism.}

% Methodology
% \textcolor{blue}{[GSG] following the KINNs notation pattern, other suggestion, letting $m$ be the number of model parameters, and $i$ as the species index.

%   \textcolor{blue}{[GSG] I think there is some confusion here. Why are there two subindices for each $\mathbf{Q}$? Could it have been $\mathbf{Q}_i^T\mathbf{Q}_j$ instead? Does it include $\mathbf{Q}_i^T\mathbf{Q}_i$? If that is the case, there should be a more efficient way to compute $V(\boldsymbol{\theta})$ as 
 %   \begin{align*}
 %       \text{let }\mathbf{R}&=\sum_i^G\sum_j^{i-1}\sigma_{i,j}\mathbf{Q}_i^T\mathbf{Q}_j,\\
 %       \mathbf{S}&=\sum_i^G\sigma_{i,i}\mathbf{Q}_i^T\mathbf{Q}_i\\
 %       V(\boldsymbol{\theta})&=\left[\mathbf{R}^T+\mathbf{R}+\mathbf{S}+\Sigma_\boldsymbol{\theta}^N\right]^{-1}
 %   \end{align*}
 %   Maybe this could be just noted in the text while pointing to the supplementary material.
 % }

 % With respect to the Fisher information matrix constructed in Equation \ref{fisherInformationMatrix}, the D-optimality is written as 

%As previously mentioned, we are exploring a synthetic oxidative propane dehydrogenation (OPDH) case study. 
%PDH and OPDH are critical processes for the production of propylene, a necessary feed-stock for plastic production, and offers a relatively complex series of reaction steps. 
%Although elementary reactions can be used in this analysis, we believe it is unnecessary to explore that level of detail and understand that all reaction steps are not going to be observable in a reactions system. 
%In catalysis, there is the added challenge of structural uncertainty in the mechanisms. 
%The divergence exploration through MBDoE is studied using these two reactions.

% Precision results
%Although we are using the models and parameters defined in the previous section, we are assuming that we do not have values for these prior to optimization. 
%For this reason, we have to select initial guesses for these parameters and choose to begin with values representing common approximations. These include -0.3 eV for the free energy of adsorption and 1 to 1.5 eV for the free energy of reaction. It is well known that initial guesses can have a major impact on the identification of global vs local optima. It is assumed that these initial guesses fall within the "global" well, but acknowledge any additional study will require further verification or the use of alternative models to reach a minimum. We also note that not all parameters are included in the optimization analysis. This is due to the limited sensitivities of some parameters in the model. To confirm which parameters can be excluded from a model momentarily, a Hessian calculation can be performed to determine the degree of sensitivity of these parameters. Many of these parameters can also be excluded due to their value in the energy space (e.g. -2.98 eV) will likely never be observed using the TAP reactor.
%To begin increasing the precision and our understanding of these parameters, we start with a simple set of experimental conditions. We do not have an initial understanding of the uncertainty, so using MBDoE immediately is less useful. 
%Comparing our fitted values from the initial experiment to the actual parameters used to simulate the experiment, we see fairly strong agreement between the two. Most parameters are within 0.03 eV of their synthetic values, with 

%Having reduced these parameters once, we should see if additional experimental data selected from MBDoE will improve it further. 

% Divergence results

%In place of generating the synthetic data using the same parameters, we made slight, random variations to the parameters and used them instead. This made divergence identification more complex and resembled a potential future application more realistic. 
%In this application, three models are assumed to have previously been identified and TAP is assumed to be an appropriate method for selecting the correct mechanism.

% Precision discussion

%In the results section, we showed that we were able to select experiments that reduced the uncertainty of the associated parameters. 

%However, this approach does not show that MBDoE is an effective method or that we are quantitatively predicting experiments to gain information. 
%The actual information gained here is defined as the determinant of the covariance matrix following optimization. 
%If MBDoE is working efficiently, we expect to observe low values of actual information with low values of predicted information. Similarly, we can observe the correlation between the predicted information and the confidence intervals of the individual parameters. Ideally, each parameter will have a gradual reduction in the uncertainty correlated with the actual information gain. 
%We fit the parameters to each of the experimental condition sets in the grid space for each step in the experiment selection process of the results, as well as quantify the uncertainty.
%To show that we are predicting useful experiments through MBDoE, we need to show that there is a correlation between the predicted and actual information gained (left subplot). The determinant of the inverted Fisher information matrix and the determinant of the covariance matrix following optimization should both be small for "optimal" experiments. This optimal experiment should also show that the confidence intervals for individual parameters are reduced most at these operating conditions (central and right subplot). }
%Now that trends based on initial conditions have been observed, the impact the optimal criteria have on reducing parameter uncertainties following re-optimization at each experiment, instead of all simultaneously in the D-optimal form, can be observed. These plots are presented in Figure \ref{}, with the confidence interval of the re-fitted parameter being presented on the y-axis. 

%The D-value and the calculated confidence intervals are also correlated, indicating the design approach adequately identifies appropriate experiments for improving this parameter. 
%, indicating this parameter is poorly defined in the system and other parameters dominate the experimental search. 
%Even though some experiments cause a significant improvement in the confidence of $\Delta{}G_{1}$, they are predicted to provide limited additional information compared to other experiments.

%Next, the free energy of adsorption of propene ($\Delta{}G_{2}$) was analyzed. Of the parameters discussed so far, this parameter is least impacted by the initial condition, although the gradual reduction in the uncertainty is still observed as the predicted D-value decreases. Some experiments result in little to no change in the confidence, but a majority of them reduced the uncertainty by a factor of 0.5 to 1. The free energies of activation of propane dehydrogenation, propane combustion, and propene combustion ($G_{a}^{3}$, $G_{a}^{4}$, and $G_{a}^{5}$, respectively) are presented in the final subplots. No outliers or surprises are found in these trends. There is the same general improvement in the confidence found for the other parameters with a few exceptions in experiments predicted to perform poorly. 
%To explore the performance of this additional application of MBDoE, similar graphs to those of Figure \ref{optimal_std_1} were generated and are presented in Figure \ref{optimal_std_2} following the second experiment. Subplot A again shows the direct comparison between the actual and predicted D-values for each experiment. Unlike the predicted D-value plot found for the first additional experiment, there is far more vertical dispersion along the predicted values. The optimal predicted experiment also only provides a mild improvement in the model compared to alternative ones, indicating there is less benefit to the experiment. There are also more experiments that outperform the predicted optimal. The results reveal even more outliers when analyzed in terms of the individual parameter confidence intervals. A few of the parameters ($Ga_{1}$, $\Delta{}G_{2}$, and $Ga_{5}$) do maintain a gradual uncertainty reduction as the predicted D-value decreases. However, other parameters fair worse and have disjointed variations in their actual D-values. $\Delta{}G_{0}$ and $Ga_{3}$ are two examples of this, each having sparse and lower confidence intervals in regions with high predicted D-value. Worst of all is the performance of $\Delta{}G_{1}$, the weakest defined parameter in the system based on the first two experiments. Although there are some experiments that have low predicted and actual D-values simultaneously, the distribution outside of these few has limited correlation. 
%Since we found that the MBDoE algorithm did not identify the optimal experiment on the third experiment and some parameters did not correlate with the predicted information, we want to test alternative design criteria to see if optimal experiments can still be identified. 
%Our primary goal is to observe a noticeable reduction in the uncertainty of our least determined parameter (i.e. $\Delta{}G^{1}$) with the hope that improving this parameter will help constrain the additional parameter. 
%Isolating the design in terms of $\Delta{}G_{1}$ addresses this issue, having little scatter around the optimal experiments and, in turn, a higher degree of stability and confidence in the result.
%The optimal experiment for $\Delta{}G_{1}$ does lead to higher confidence intervals for $\Delta{}G_{0}$ and $Ga_{3}$, but these appear to be more confident values considering the smooth, continuous nature of the trends in all subplots near this region. Focusing the DoE on a single poorly-determined parameter is an effective strategy to reduce the uncertainty on that parameter, especially in the case that the full design of experiments does not significantly reduce uncertainty.

% Divergence discussion

%will have a strong overlap between the two and that there is a benefit to designing experiments to help avoid these regions.

%The analysis presented in the results section shows that MBDoE is capable of identifying experiments with a maximal difference and may be required to identify the correct mechanism. This is especially true in the case where kinetic parameters are expected to vary minimally between experiments. However, the analysis assumes that the rate constants obtained from fitting to the initial experiment are held constant and not re-fitted to the second experiment. In a real scenario, a researcher would likely want to re-fit the model to both experiments to determine whether their kinetic model structure was capable of explaining all the observed data. For this reason, mechanisms 1 and 2 were re-optimized to the experimental data generated during the grid search. This analysis is presented in Figure \ref{opt_divergence}. It is clear that after re-optimization the BIC is not correlated to the divergence, and discriminating between the two mechanisms is not possible at any of the experimental conditions explored. There are some experiments where small differences are observable, but they are scattered randomly throughout the divergence and are too narrow to draw any strong conclusions. The prior optimal experiments for each divergence criterion do not perform well visually either (see Figure \ref{opt_flux}). These results suggest that the convolution of parametric and structural uncertainty presents a significant challenge since it is not possible to distinguish between mechanisms if the parameters are only obtained by fitting to the kinetic data. 

%they are not compatible in their current form, primarily due to the high degree of flexibility present in the mechanisms. This flexibility leads to mechanisms that can describe a broad range of experiments following optimization. Providing the MBDoE workflow with additional experimental data sets could help alleviate these issues.  

%\subsection{Refining the design of experiments and alternative applications}



%An alternative challenge in TAP outside of catalysis is separations. The intrinsic properties of separation materials and the sensitivity of the transport processes have seen some exploration over the years, but to a lesser degree \cite{keipert1998determination,shostak2022parametric}. Although exploring these materials is a complex endeavor, it can be seen as less challenging than understanding the pool of adspecies on catalytic materials. The parameters inherent in separation/adsorption processes can be improved using the MBDoE. Robust implementations involving both discrimination and precision could even be implemented with more confidence, establishing a set of common separation models to automatically explore \cite{bawa2022rapid}. More general forms of MBDoE could be useful in this endeavor \cite{wang2022pyomo}. 

%Last, alternative forms for identifying optimal experiments should be explored. For example, Bayesian experimental design (BED) can help identify these experiments while making fewer assumptions about the uncertainty space (i.e. non-Gaussian distributions) \cite{savara2020chekipeuq,walker2020chekipeuq}. Robust forms of information gain (REIG) are also being developed, which could further refine proposed mechanisms \cite{go2022robust}. The primary issue is balancing utility and efficiency, where these alternative approaches typically provide the best additional experiment but can be more computationally expensive by orders of magnitude compared to MBDoE. These methods should be studied more to determine their utility with respect to TAP experimentation.

 % Conclusion
 %Variations to the design criteria did result in a more favorable identification of this parameter and could suggest a path forward for best constraining a proposed mechanism. 
